DefunT: A Tool for Automating Termination Proofs by Using the Community Books (Extended Abstract)

We present a tool that automates termination proofs for recursive definitions by mining existing termination theorems.

==> eptcsdata.tex <==
\providecommand{\firstpage}{161}
\providecommand{\publicationstatus}{Shilpi Goel and Matt Kaufmann (Eds.):\\
ACL2 Theorem Prover and its Applications (ACL2-2018)\\
EPTCS 280, 2018, pp.\ \pageref*{FirstPage}--\pageref{LastPage},
doi:\href{http://dx.doi.org/10.4204/EPTCS.280.12}{10.4204/EPTCS.280.12}}

